Empirical Risk Minimization for Time Series: Nonparametric Performance Bounds for Prediction

Empirical risk minimization is a standard principle for choosing algorithms in learning theory. In this paper we study the properties of empirical risk minimization for time series. The analysis is carried out in a general framework that covers different types of forecasting applications encountered in the literature. We are concerned with 1-step-ahead prediction of a univariate time series generated by a parameter-driven process. A class of recursive algorithms is available to forecast the time series. The algorithms are recursive in the sense that the forecast produced in a given period is a function of the lagged values of the forecast and of the time series. The relationship between the generating mechanism of the time series and the class of algorithms is unspecified. Our main result establishes that the algorithm chosen by empirical risk minimization achieves asymptotically the optimal predictive performance that is attainable within the class of algorithms.

==> abstract.tex <==
Empirical risk minimization is a standard principle for choosing algorithms in learning theory. 
In this paper we study the properties of empirical risk minimization for time series,
introducing a general framework that allows to study different types of applications that includes ARMA and GARCH forecasting as special cases.
A class of recursive algorithms is available to forecast 1-step-ahead a univariate time series generated by a parameter-driven process.
The algorithms are recursive in the sense that the forecast produced in a given period is a function of the lagged values of the forecast and of the time series.
A key feature of the analysis is that the relationship between the time series and the class of algorithms is unspecified.
Our main result establishes that the algorithm chosen by empirical risk minimization achieves asymptotically the optimal predictive performance that is attainable within the class of algorithms considered.
This implies that ARMA/GARCH forecasting based on the standard Gaussian maximum likelihood estimator achieves asymptotically the optimal predictive performance even when the conditional mean/conditional variance equation of the model is misspecified.

